Towards Carbon Footprint-Aware Recommender Systems for Greener Item Recommendation

The commodity and widespread use of online shopping are having an unprecedented impact on climate, with emission figures from key actors that are easily comparable to those of a large-scale metropolis. Despite online shopping being fueled by recommender systems (RecSys) algorithms, the role and potential of the latter in promoting more sustainable choices is little studied. One of the main reasons for this could be attributed to the lack of a dataset containing carbon footprint emissions for the items. While building such a dataset is a rather challenging task, its presence is pivotal for opening the doors to novel perspectives, evaluations, and methods for RecSys research. In this paper, we target this bottleneck and study the environmental role of RecSys algorithms. First, we mine a dataset that includes carbon footprint emissions for its items. Then, we benchmark conventional RecSys algorithms in terms of accuracy and sustainability as two faces of the same coin. We find that RecSys algorithms optimized for accuracy overlook greenness and that longer recommendation lists are greener but less accurate. Then, we show that a simple reranking approach that accounts for the item's carbon footprint can establish a better trade-off between accuracy and greenness. This reranking approach is modular, ready to use, and can be applied to any RecSys algorithm without the need to alter the underlying mechanisms or retrain models. Our results show that a small sacrifice of accuracy can lead to significant improvements of recommendation greenness across all algorithms and list lengths. Arguably, this accuracy-greenness trade-off could even be seen as an enhancement of user satisfaction, particularly for purpose-driven users who prioritize the environmental impact of their choices. We anticipate this work will serve as the starting point for studying RecSys for more sustainable recommendations.

==> 3_data_repo1.tex <==

\begin{wrapfigure}{r}{0.5\textwidth}
\vskip-.9cm
\begin{minipage}{80mm}
  % \centering
  \raggedleft
\begin{align*}
    % \begin{split}
         & \texttt{user id:} ~~~~56,680&\\
         & \texttt{rating:} ~~~~5&\\
         & \texttt{date:} ~~~~2006-11-11&\\
         & \texttt{review:} ~~~~\texttt{Great!}&\\
         & \texttt{recipe id:} ~~
            \begin{cases}
              \texttt{recipe name:} & \texttt{patato}\\
              \texttt{ingredient ids:} & [2851,\ldots]\\
              \texttt{CO$_2$ footprint:} & 4.46 \\
              \texttt{ingredient names:} & [\texttt{onion},\ldots]\\
              \texttt{ingredient quantities:} & [1,\ldots] \\
              \texttt{greenness:} & 3.37
            \end{cases}  &
    % \end{split}
\end{align*}
\captionof{figure}{An example of an entry in the RecipeEmission dataset. }
        \label{recipe_entry}
\end{minipage}
  \vskip-.5cm
\end{wrapfigure}

%PREAMBLE
\textcolor{blue}{In this section, we present the properties and statistics of our prepared RecipeEmission dataset and answer RQ1. Then, we describe our data preparation process.} Our initial data come from the Food.com dataset in \cite{majumder2019generating}, which contains users interacting with recipe items via explicit ratings and textual reviews. Each recipe has its name and list of ingredients as a feature. As additional features, we mined the ingredient quantities, \emph{the CO$_2$ equivalent} (CO$_2$-eq) of the recipes and their greenness. Greenness is a quantization of the CO$_2$-eq into a finite scale of real-valued scores. An example of an entity is shown in Fig.~\ref{recipe_entry}. %In this section, we first present the steps followed to build the RecipeEmission dataset in Sec.~\ref{subsec:buildData}.

%SUBSECTION
\subsection{Building the Dataset}\label{subsec:buildData}


We build the RecipeEmission dataset from the Food.com (the original) dataset present in \cite{majumder2019generating} by adding the CO$_2$-eq and greenness to the different recipe items. We break each recipe down into its ingredients (present in the original dataset) and the respective quantities (not present in the original dataset). Upon scraping the ingredient quantities and the CO$_2$-eq, we compute the recipe CO$_2$-eq as a weighted sum of those of the ingredients. This task presents the following intertwined challenges: 
%
\begin{itemize}
\item[--] \emph{high interaction sparsity:} the original dataset is sparse ($99.998\%$) and often it contains a few interactions per user or item; this leads to some recipes being rated only by one user and to some users having rated only one recipe;
\item[--] \emph{missing ingredient quantities:} quantities of the ingredients are not present in the original dataset and need to be found differently;
\item[--] \emph{non-unified description:} descriptions of the quantities differ (e.g., 1-2 cups, 1.5 grams) and they are often expressed in qualitative terms (1 piece, a pinch);
\item[--] \emph{lack of CO$_2$-eq consensus:} there is no standard and unified repository to find the CO$_2$-eq of the different ingredients (this differs from the country of origin, the technology used to harvest them, transportation to destination, and season); this often requires extensive manual work;
\item[--] \emph{missing CO$_2$-eq values:} CO$_2$-eqs are missing for particular ingredients, leading to recipes having only some ingredients for which the CO$_2$-eq could be found.
\end{itemize}
%
Here, we present the methods pursued to address these challenges. These methods consider the thin balance between \emph{including as many interactions as possible} and \emph{having reliable CO$_2$-eq measures} for the items. Our focal principle is to preserve the key properties (see Fig.~\ref{fig:dataset_props}) and statistics (see Table~\ref{tab_stat}) of the original dataset to ensure that they remain comparable to baselines. The methods are composed of five steps: $i)$ pre-filtering the data; $ii)$ quantifying the ingredients in the recipes; $iii)$ quantifying the CO$_2$-eq; $iv)$ quality assessment; $v)$ quantizing the CO$_2$-eq. Fig.~\ref{fig:dataset_building} provides a high level overview of the process of building the dataset.

\begin{figure}
  \includegraphics[width=\textwidth]{Figures/dataset_building.pdf}
  \caption{Overview of the steps taken to build the dataset. First of all, pre-filtering is performed, followed by ingredient and CO$_2$-eq quantification. Finally, the CO$_2$-eq values are transformed to a greenness scale.}
  \label{fig:dataset_building}
\end{figure}

%%%% PREFILTERING
\smallskip
\noindent\textbf{Pre-filtering.} The long-tail distribution of the Food.com dataset (see Fig.~\ref{fig:dataset_props}) implies that we need to find the CO$_2$-eq for some items that play a minor role in assessing the overall performance of a RecSys algorithm\footnote{These items would, however, be relevant if we were interested in addressing the (strict) cold start problem for RecSys. But since our focus is on assessing the \emph{greenness} of RecSys algorithms as a whole, we can ignore these items. Typically, these interactions are treated as spurious or erroneous and are removed.}. To reduce the number of recipes for which the CO$_2$-eq has to be found, we filtered out the items and users with a few interactions as commonly done in RecSys datasets --e.g., MovieLens filters on the minimum number of interactions per user~\cite{harper2015movielens}. Specifically:
%%%%%%%
\begin{enumerate}[label=\arabic*)]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\item We removed all recipes having less than $20$ ratings.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\item From the remaining recipes, we removed those for which not all ingredients could be found.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\item Further, we removed all users that had no interaction with the remaining recipes.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\item From the recipes with more than $20$ interactions, we removed those users that have rated only that recipe, while still maintaining at least $20$ interactions per recipe.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\item {Finally, we removed those recipes for which all users have rated less than 20 recipes on average. That is, for each recipe, we extracted the user IDs of users who have interacted with the recipe and measured their total number of interactions. Then, we removed those recipe items for which the respective users rated less than 20 items. The latter helps us remove recipes that occur only in sparse parts of the dataset and tackle the cold start issues.} %\red{@Raoul: check what I wrote here based on our long-time ago discussion. I recall though there you were talking about "averages". Could you explain it here and update this part accordingly?} 
This led to the final RecipeEmissions dataset reported in Table~\ref{tab_stat}.
%
%\blue{Finally, we also removed recipes for which all users rated less than 20 recipes on average.}\red{EI: I don't get this! Does it mean we removed those recipes that had again less than $20$ ratings?} \green{Explanation: first we removed all recipes with less than 20 ratings (so less than 20 users). Later on, we removed also recipes for which its \emph{users} had less than 20 ratings \emph{on average}. In other words, we calculate the average number of interactions among users of every recipe and we remove all recipes for which this is less than 20. We discussed this a long time ago, and the main reason we did this, was to remove recipes that only occured in very sparse parts of the dataset. We figured this would be likely to not change the results much, while at the same time it would cost much to find their CO2.}\red{EI: Still unclear to me! We need to talk about this; so you can explain it to me in 5 min.} This led to the final RecipeEmissions dataset reported in Table~\ref{tab_stat}.
\end{enumerate}

%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%% TABLE
\definecolor{Gray}{gray}{0.9}
\begin{table}[t]
\caption{Ingredient categories, their representations, and their corresponding weights conversion from pint, cup, teaspoon, and tablespoon to grams. "na." implies that measuring approach was not present for the specific category. The "pinch" metric was used for spices and salt and we choose salt as the representative ingredient with a conversion rate of 0.36 grams.}
\label{tab:my-table-conv}
\begin{tabular}{lccccc}
\hline\hline
\rowcolor{Gray}
{\textbf{Category}}     & \textbf{Represented by} & \textbf{Pint-to-g} & \textbf{Cup-to-g} & \textbf{Teaspoon-to-g} & \textbf{Tablespoon-to-g} \\
{liquids}               & water                   & 473.18   & 236.59   & 4.93 & 14.79         \\
\rowcolor{Gray}
{sugars and sweeteners} & raw sugar               & 414.02   & 227.36  & 4.74  & 14.21        \\
{flours}                & all-purpose flower      & 250.31   & 125.16 & 2.61 & 7.82         \\
\rowcolor{Gray}
{oils and fats}         & olive oil               & 434.38    & 217.66   & 4.53  & 13.6       \\
{spices}                & cinnamon                & 264.98   & 132.49  & 2.76  & 8.28         \\
\rowcolor{Gray}
{nuts}                  & almonds                 & 217.66     & 108.83  & na.  & na.       \\
{fruits and vegetables} & onion                   & 104.10  & 150    & na.  &na.      \\
\hline\hline
\end{tabular}
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%

%%%% QUANTIFY INGREDIENTS
\smallskip
\noindent\textbf{Quantifying ingredients.} The original dataset from \cite{majumder2019generating} does not contain the ingredient quantities, which we got from Food.com:
%%%%%%%%%%%%%%%
% ENUMERATE
\begin{enumerate}[label=\arabic*)]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\item \emph{Scrape:} We scraped Food.com using the URL:
\begin{center}
\emph{www.food.com/[tag]/[recipe name]-[recipe id]}.\smallskip\\ 
\end{center}
Here \emph{[tag]} is \emph{recipe} or \emph{about} depending on the recipe. The \emph{[recipe name]} is comprised of the decapitalized version of the recipe name with spaces replaced by hyphens (-). The \emph{[recipe id]} is also available in the original dataset.
%
All ingredients on Food.com have unique identifiers, but those do not always correspond to the identifiers in the original dataset. However, the order of ingredients on Food.com follows that in the lists. We contrasted the list lengths and the ingredient names to find the corresponding entities, and we also checked this manually for $50$ random recipes. Thus, we scraped the ingredient quantities and respective units in their default order from Food.com. \smallskip

For 797 recipes, the ingredient list on Food.com contained more ingredients than the list in the original dataset. These additional ingredients formed alternatives or minor additions that do not change the recipe. We checked if the names of the ingredients in the original dataset were contained in the names of scraped ingredients. If so, we matched the two and retrieved the respective quantities; otherwise, we considered the scraped ingredient not to be present in the original dataset and removed the ingredient.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\item \emph{Standardization:} The quantities on Food.com are expressed in different forms (e.g., range 1-2 cups; decimal format 2.5 cups; decimal fractions 2 1/2 cups) and in different units (grams, ounce, pinch). We standardized the quantities into a decimal format and in grams to allow for an easier CO$_2$-eq conversion, which is expressed in Kg. The conversion rates are reported in Table~\ref{tab:my-table-conv}.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\item \emph{Manual completion:} To estimate the weight of ingredient instances in non-standard quantities (e.g., "two chicken breasts," "a bunch of cabbage," or "a handful of cabbage"), we engaged four student annotators from diverse demographic and cultural backgrounds. Each annotator was tasked with determining the weight in grams of various ingredient-measure combinations sampled from our dataset. They were instructed to search for the ingredient and measure combination on Google.com and record the first relevant result they found. Additionally, they were asked to provide their source and rate their confidence in the accuracy of their findings on a scale from 1 to 10 to support the verification process. To enhance efficiency and consistency, we provided custom software that allowed annotators to input both their results and confidence levels directly. The software randomly assigned ingredient-measure combinations, and each annotator processed half of the dataset, ensuring all ingredients were annotated multiple times.

Each of the 4,010 non-standard ingredient instances was annotated. Estimates with confidence ratings below 5 were re-examined, leading to 73 re-annotations. To assess inter-rater reliability, we calculated the mean absolute difference between annotations from different raters, which revealed a disagreement of a mere 2\%, indicating a high level of reliability.
%\textcolor{red}{An annotator estimated the weights for each of the $4.010$ ingredient instances that were in non-standard quantities and with repetition (e.g., two chicken breasts, a bunch of cabbage, or a handful of cabbage) by assigning it to the first search result on Google.com. 
%We found the quantities for \blue{$4.010$} ingredients which were in non-standard quantities (e.g., two chicken breasts or one bell pepper). A manual annotator estimated the weights of each ingredient by assigning it to the first search result on Google.com. 
%Annotators also provided the source and a numerical value (1-10) of how certain they were about the correctness of the annotation. Annotations with certainties below $5$ were re-inspected, resulting in $73$ re-annotations. \textcolor{blue}{Moreover, as a measure of the inter-rater reliability, we calculated the mean absolute difference between the annotations of the different raters. This showed a mere $2\%$ disagreement between annotators, indicating a high reliability of annotations}}
\end{enumerate}


%%%%%QUANTIFYING-CO2
\smallskip
\noindent\textbf{Quantifying CO$_2$-eq.} Aided by the list of ingredients, the respective quantities, and the standardized units, we found the CO$_2$-eq of the $2735$ unique ingredients as follows: %\blue{$2735$}\footnote{\red{EI: above we have 4010 ingredients in non-standard quantities but we also had other ingredients, which if I'm not wrong were quite a few? Can we give that all number somewhere? But where we say we found the co2-eq for 2735 ingredients. So, one would ask what happened to the remaining ones. We shall mention somewhere this!} \green{I am not sure I was clear here: there is a number of ingredients, i.e. 2735, but the ingredients are used in different instances. So, we have the ingredient cabbage, for example. Cabbage has a fixed greenness value per kg. But, cabbage is used in different instances (so, a pack of cabbage, a bunch of cabbage, and a handful of cabbage. That is why there are more instances (i.e... 4010 non-standard ones) than ingredients.)}} ingredients as follows:
%%%%%%%%%%%%%%%
% ENUMERATE
\begin{enumerate}[label=\arabic*)]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\item \emph{Ingredient filtration:} First, we removed $705$ ingredients present in quantities smaller than $50$ grams. These ingredients are in small relative quantities or have a low CO$_2$-eq, such as spices and flavorings \cite{marie_2022, marie_2022_2}. The threshold of $50$ grams is chosen as that of having a low impact on the whole recipe CO$_2$-eq, since in many recipes, the overall CO$_2$-eq is governed by a few ingredients present in large quantities and with a large carbon footprint (e.g., meat products).%, the threshold of $50$ grams is qualitatively chosen as that of having a relatively low impact on the whole recipe CO$_2$-eq.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\item \emph{Automated search:} We searched the CO$_2$-eq of all ingredients on healabel.com. This source, which provides the most extensive list of ingredients with CO$_2$-eq data, aggregates information from books, journals, and validated online articles, including the FDA's Food Resources for Consumers, the World Health Organization, and the US Department of Agriculture. Having an extensive collection of CO$_2$-eq, this website also allowed a consistent measure across the different items in the dataset. We extracted the CO$_2$-eq via the ingredient names using the URL:
\begin{center}
\emph{https://healabel.com/ [first letter ingredient] / [ingredient name]}.
\end{center}
Multiple word names are separated with a hyphen (-). We searched ingredients both in their singular and plural forms (e.g., nut and nuts) as both were present. Several ingredients are variations of others (e.g., red pepper, green pepper) and have comparable CO$_2$-eq. So, we removed the adjectives and searched their stem form (e.g., pepper). For some composite words, the adjective represents the main ingredient (e.g., meat substitute). {However, for such ingredients, it is inaccurate to use the adjective to find the CO$_2$-eq. For example, a meat steak differs from a meat sauce. Thus, we found the CO$_2$-eqs of these ingredients manually.}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\item \emph{Manual search:} We searched the CO$_2$-eq first on healabel.com to standardize the data as much as possible and then in literature. The latter is achieved by searching on Google Scholar using the query \emph{ [ingredient name] CO$_2$ footprint} and retrieving the CO$_2$-eq from the most cited paper. The papers used for this step are \cite{yuttitham2011carbon, sevenster2008sustainable, dalla2017environmental, fantozzi2019life, parajuli2021cradle, taylor2014greenhouse, vasilaki2016water, pelletier2013carbon, espinoza2011carbon}.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\end{enumerate}

%%%%QUALITY CHECK
\smallskip
\noindent\textbf{Quality assessment.} To evaluate the quality of the dataset, $100$ random ingredients were selected, and the accuracy of their retrieved CO$_2$-eq was manually inspected. Due to the complexity of this process, we evaluated the similarity between the ingredient name and the corresponding name used to retrieve the CO$_2$-eq. For example, retrieving the exact CO$_2$-eq value for the ingredient "1 cup of shredded bell pepper" is a complex task, or in some cases, even impossible. Hence, we tackled this issue by retrieving the CO$_2$-eq value for the most similar ingredient to "1 cup of shredded bell pepper" with a known CO$_2$-eq. In this case, the ingredient "bell pepper" would be the best option. The resulting accuracy of this evaluation was $92\%$, indicating that for $92\%$ of the ingredients, we could accurately retrieve the CO$_2$-eq value. We deemed this accuracy satisfactory as we are not interested in the precise CO$_2$-eq but in relative quantification. A more precise quantification should start by standardizing the quantities of the different ingredients, their densities, the dynamics of CO$_2$-eq (season, distance from the user), and the sources from which the CO$_2$-eq is retrieved. This by itself requires extensive separate research.\footnote{The complexity arises from the lack of global standardization in CO$_2$-eq and weight conversions for ingredients. For example, the conversion rate for \emph{a portion of beef} differs substantially between Texas and the Netherlands. Factors such as the breed and age of the animal further complicate this. Therefore, constructing a unified dataset for detailed CO$_2$-eq analysis would require extensive interdisciplinary research, which goes beyond the scope of a single paper.}

%%%%%GREEN CONVERSION
\smallskip
\noindent\textbf{Green conversion.} Each of the above steps introduces some uncertainty to the precise CO$_2$-eq of whole recipes. Factors contributing particularly to this uncertainty include the precise weight calculation of the ingredients, manual annotations, removal of the ingredients with small quantities, variations in ingredient names, accuracy of CO$_2$-eq retrieval, and the sampling used in quality assessment. To reduce the effect of this uncertainty and to be consistent with the interval of rating values, we transformed the CO$_2$-eq into \emph{greenness} values at the interval $[0, 5]$, where a low value corresponds to a less green item (high CO$_2$-eq) and a high value to a greener item (low CO$_2$-eq).
%
%The CO$_2$-eq in Kgs of the retried recipes have an uncertainty around the indicated value because of the tedious task of finding a unified way of quantifying the CO$_2$-eq. To reduce the effect of this uncertainty, we quantized the CO$_2$-eq into a discrete interval as done for explicit ratings. More precisely, we quantized the CO$_2$-eq into \emph{greenness} values in the interval $\{0,\ldots, 5\}$, where a low value indicates a less green item (high CO$_2$-eq) and a low value a greener item (low CO$_2$-eq). This greenness conversion is done so that the interval matches that of the ratings and also has a similar ascending order for a more "useful item" (high rating, high greenness). 
%
Specifically, denoting the CO$_2$-eq of item $i$ by $c_i$, the greenness $g_i$ is defined as
%
\begin{equation}\label{eq_greenness}
g_i = \ccalQ\left[\log\left(1+ \frac{1}{c_i}\right)\right]
\end{equation}
%
where the inverse ensures that items of low CO$_2$-eq are greener and vice versa; the logarithm amortizes the exponential decay spreading of the CO$_2$-eq; and $\ccalQ[\cdot]$ is a function that projects the greenness values into $[0, 5]$ interval, e.g., values higher than 5 are mapped to 5. We added a one within the logarithm to have only positive values inspired by the tf-idf weighting \cite{salton1988term}. This greenness conversion matches that of the ratings and has a similar ascending order for a more "useful item" (high rating, high greenness).
%
%\blue{Another effect of the logarithm is that it also reduces the uncertainties around the found CO$_2$-eq.}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%   STATISTIC TABLE
\begin{figure*}[!tp]
\centering
\begin{subfigure}{.33\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{Figures/user_rankvsrating.pdf}
  \caption{}
  \label{fig:sub_user_rank}
\end{subfigure}%
%
\begin{subfigure}{.33\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{Figures/item_rankvsrating.pdf}
  \caption{}
  \label{fig:sub_item_rank}
\end{subfigure}
%
\begin{subfigure}{.33\textwidth}
\centering   \includegraphics[width=1\linewidth]{Figures/rating_distro.pdf}
\caption{}
\end{subfigure}
%
%\caption{Long-tail distributions of the RecipeEmission and other datasets. (a) User engagement distribution (total ratings of each user). The RecipeEmission dataset has a similar distribution as the starting Food.com dataset and baselines. There are no users with a large number of ratings because of the filtration steps over the minimum number of interactions per item. (b) Item popularity distribution (total ratings of each item). The distribution of the RecipeEmission dataset follows closely that of the original Food.com. MovieLens datasets filter on the minumum number of interactions per user which can be noted by the trunkated distributions in this panel.}
\caption{Distribution of the statistics for the RecipeEmission and conventional datasets. \textbf{(a)} Long-tail distributions of the user engagement (total ratings of each user). RecipeEmission has a similar distribution as the starting Food.com dataset and baselines. There are no users with a large number of ratings because of the filtration steps over the minimum number of interactions per item. \textbf{(b)} Long-tail distributions of the item popularity distribution (total ratings of each item). RecipeEmission closely follows the distribution of the original Food.com. MovieLens datasets are filtered on the minimum number of interactions per user which can be noted by the truncated distributions in this panel. \textbf{(c)} Rating distribution scaled to the set $\{1, \ldots, 5\}$. All datasets but Book-Crossing have a skew towards high rating values. RecipeEmission respects the distribution of the original Food.com dataset, which follows a similar pattern as the MovieLens datasets.}
\label{fig:dataset_props}
\end{figure*}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table*}[!t]
\centering
\caption{Dataset statistics. RecipeEmission has a comparable sparsity to the baseline datasets. The reduced number of users and items is a result of the filtration steps to improve the efficiency in finding the CO$_2$-eq of the ingredients. We also see a high average rating in both RecipeEmission and Food.com, which needs to be accounted for when comparing the algorithms.}
\label{tab:dataset-comparison}
\resizebox{\textwidth}{!}{%
\begin{tabular}{l c c c c c}
\hline\hline
                                                                             & \textbf{RecipeEmission} & Food.com & Movielens100k~\cite{harper2015movielens} & Movielens1M~\cite{harper2015movielens} & Book-Crossing~\cite{ziegler2005improving} \\ 
                                                                          \rowcolor{gray!50}
\#users                                                                      & 32.090           & 226.570   & 943           & 6.040        & 105.283        \\ 
\#items                                                                      & 5.595            & 231.637   & 1.682          & 3.706        & 340.556        \\ 
\rowcolor{gray!50}
\#interactions                                                               & 247.219          & 1.132.367  & 100.000        & 1.000.209     & 1.149.780       \\ 
sparsity                                                                     & 99.86\%         & 99.998\% & 93.70\%       & 95.53\%     & 99.997\%      \\ 
\rowcolor{gray!50}
rating values                                                               & \{0,\ldots, 5\}               & \{0,\ldots, 5\}         & \{1,\ldots, 5\}              & \{1,\ldots, 5\}            & \{0,\ldots, 10\}             \\ 
average rating (std.)                                                               & 4.57 ($\pm 1.054$)           & 4.41 ($\pm 1.26$)    & 3.53 ($\pm 1.13$)          & 3.58 ($\pm 1.12$)       & 2.87 ($\pm 3.85$)         \\ 
\rowcolor{gray!50}
med. interaction per item $\backslash$ user & 27$\backslash$3              & 2 $\backslash$ 1       & 27 $\backslash$ 65            & 124 $\backslash$ 96         & 1$\backslash$1 \\
\rowcolor{gray!50}
%\begin{tabular}[c]{@{}l@{}}median interactions\\ per item $\backslash$ user\end{tabular} & 27$\backslash$3              & 2 $\backslash$ 1       & 27 $\backslash$ 65            & 124 $\backslash$ 96         & 1$\backslash$1              \\ 
\hline\hline
%\begin{tabular}[c]{@{}l@{}}median interactions \\ per user\end{tabular}      & 3               & 1        & 65            & 96          & 1             \\ \hline\hline
\end{tabular}}
\label{tab_stat}
\end{table*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% In this section, we present the properties and statistics of the prepared RecipeEmission dataset.

% \smallskip
% \noindent \textbf{Outline of the methods.} Building the RecipeEmission dataset posed several challenges, such as: i) a high sparsity ($99.998\%$); ii) ingredient quantities missing or described in different ways (cups, graphs, piece); iii) no standardized and unified repository to identify the CO$_2$-eq of an ingredient; iv) CO$_2$-eq values being unknown for some ingredients. To keep the discussion concise, we outline the main steps of building the dataset in the sequel and defer the details to Sec.~\ref{subsec:buildData}. 

% \textcolor{blue}{Our approach to addressing these challenges was to retain as many interactions as possible from the original dataset while ensuring reliable CO$_2$ estimates. We also aimed to preserve the original dataset’s properties and statistical characteristics.} Thus, we proceeded in three steps. First, we filtered out recipes with a single rating to limit the search for the carbon footprint to the most relevant entries and we removed recipes for which ingredients were missing. \textcolor{blue}{This was done to ensure a high-quality subset for subsequent CO$_2$ estimation.} Second, we scraped the ingredient quantities from the website Food.com and standardized measurements to grams for ingredients originally listed in qualitative terms (e.g., pieces or a pinch). \textcolor{blue}{To achieve this, manually crowdsourced annotations were collected for around 4,000 ingredients.} Third, we quantified the CO$_2$-eq of recipes through a combination of automated and manual searches across online repositories and scientific publications.

% A quality assessment of the resulting dataset was performed in two directions. First, the dataset statistics were compared to those of the original Food.com-based dataset as shown in Fig.~\ref{fig:dataset_props} and Table~\ref{tab_stat}. Second, 100 random ingredients were taken, and their retrieved CO$_2$-eq was re-inspected, \textcolor{blue}{the annotation process and quality assessment are detailed in Sec.~\ref{subsec:buildData}}. We found an accuracy of $92\%$, whereas we observed little changes for the remaining ones. \textcolor{blue}{Finally, considering that the dataset contains many recipes with relatively low CO$_2$-eq values, we derived the greenness values by applying a logarithmic function on CO$_2$-eq values to smooth out large variations (see Eq.~\eqref{eq_greenness}). The result is a greenness distribution where larger values imply greener items.}

\subsection{Dataset statistics} 

RecipeEmission has $32.093$ users, $5.605$ recipes, and $247.521$ interactions, modelled as explicit ratings $\{0,\ldots,5\}$ leading to a sparsity of $99.86\%$. Figs.~\ref{fig:dataset_props}(a) and~\ref{fig:dataset_props}(b) show that RecipeEmission preserves key properties of conventional RecSys datasets such as the long-tail distribution of both user engagement --most user engage with few items-- and item popularity --a few items collect most ratings.

Table~\ref{tab_stat} contrasts the statistics of these datasets. RecipeEmission has fewer users, items, and interactions than Food.com. This is the result of the performed filtration steps to ease the mining the CO$_2$-eq, which also remove noisy/spurious interactions. That is, many users have a few interactions with the items, as shown also in the last row of Table~\ref{tab_stat}. Hence, we selected only recipes with at least $20$ ratings while still preserving the long-tail distribution and a sparsity greater than 99.8\%, in order to retain comparability with conventional RecSys datasets.

RecipeEmission has an average rating of $4.57$, which is close to its maximum of five. This is inherited from the ratings present in the original Food.com dataset. To illustrate the latter, Fig.~\ref{fig:dataset_props} (c) shows that the rating distributions of these two datasets and those of the baselines are similar and skewed towards higher values. Consequently, this skewness will bias the predicted recommendations towards high values. That is, the predicted ratings will have a lower spread which may lead to similar accuracies when comparing different RecSys algorithms. Thus, a relative comparison w.r.t. a baseline algorithm is more insightful to draw conclusions than focusing on absolute numbers. We shall elaborate on the latter in Sec.~\ref{sec:results}.

\begin{figure}[!tp]
\centering
\begin{subfigure}{.4\textwidth}
  \includegraphics[width=1\linewidth]{Figures/user_item_co2.pdf}
  \caption{}
  \label{fig:user_item_co2}
\end{subfigure}%
\centering
\begin{subfigure}{.4\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{Figures/user_item_greenness.pdf}
  \caption{}
  \label{fig:user_item_greenness}
\end{subfigure}%
\vspace{\floatsep}
\begin{subfigure}{.4\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{Figures/emissions_per_rating.pdf}
  \caption{}
  \label{fig:emissions_per_rating}
\end{subfigure}%
\begin{subfigure}{.4\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{Figures/greenness_per_rating.pdf}
  \caption{}
  \label{fig:greenness_per_rating}
\end{subfigure}%
\caption{Emission distributions of RecipeEmission dataset. \textbf{(a)} CO$_2$ values of users and items. The high CO$_2$-eq outliers are again the result of recipes with large quantities of high-CO$_2$ products. \textbf{(b)} greenness distributions of RecipeEmissions dataset \textbf{(c)} Distribution of emissions per rating. The large number of outliers is caused by the long-tail distribution of CO$_2$ values of recipes. \textbf{(d)} Greenness distributions over the rating values. There is no apparent distribution shift to the rating, indicating that users did not account for the item greenness when rating them.}
\label{fig:co_rank_rating}
\end{figure}


%
% \smallskip
\subsection{CO$_2$-eq distribution} 
Fig.~\ref{fig:user_item_co2} shows the CO$_2$-eq distributions of the recipes and users at the interval $[0, 200]$ Kg. Most recipes have a small footprint, and most users interact with recipes with a lower footprint. The decay of these curves indicates a long-tail CO$_2$-eq distribution similar to that of ratings. High CO$_2$-eqs are typically associated with items containing large quantities of high-CO$_2$ ingredients, such as meat products. Most recipes do not contain such high quantities, leading to a low CO$_2$-eq. Thus, the greenness of different recommender systems in absolute terms is unlikely to differ much. 
Analogously, Fig. \ref{fig:user_item_greenness} shows the greenness distribution for the recipes and users. The recipes are skewed towards greener values and, similarly, users interact mostly with greener items. 

Fig. \ref{fig:emissions_per_rating} shows the recipe CO$_2$-eq distribution w.r.t. the ratings. We observe no apparent difference between the distributions, indicating the recipes' carbon footprint plays a minor role in the ratings. 
This is a satisfactory observation, as the distribution of CO$_2$-eq values with respect to the distribution of rating values is unbiased, ensuring it does not interfere with our experimental analysis. For instance, if items with higher CO$_2$-eq values tended to receive higher ratings (e.g., 5 stars), the RecSys model could suffer from a positivity bias~\cite{huang2024going}, leading it to over-recommend these high-rated items. Such a bias would not only skew recommendation quality but also compromise the accuracy of our sustainability analysis by favoring certain groups of items. However, as shown in Fig.~\ref{fig:emissions_per_rating}, our data does not exhibit this correlation, allowing us to conduct both recommendation and greenness analysis without concern for bias related to CO$_2$-eq values. Lastly, in Fig. \ref{fig:greenness_per_rating}, the greenness distribution w.r.t. the ratings is shown. Similarly to the CO$_2$-eq, there is no strong difference between greenness values for different ratings, indicating that users did not consider greenness when rating items.






























==> data_process_diagram_.tex <==
% \documentclass[tikz,border=9pt]{standalone}
\usetikzlibrary{shapes, arrows.meta, positioning}
% \begin{document}
\begin{figure}
% \begin{minipage}{.1\textwidth}
\begin{tikzpicture}[
    box/.style={
        rectangle, draw, rounded corners, text width=2.5cm, align=center,
        minimum height=3cm, inner sep=0pt
    },
    arrow/.style={
        -{Latex[length=3mm]}, thick
    },
    scale=0.3
]
% Define nodes aligned by their top edge using anchor=north
\node[box, anchor=north, fill=blue!20] (prefilter) at (0,0) {%
    \scriptsize\textbf{Pre-filtering} \\[1mm]
    \tiny
    1. Remove users and items with limited interactions
};

\node[box, anchor=north, fill=green!20] (quantIngredients) at ([xshift=12cm] prefilter.north) {%
    \scriptsize\textbf{Quantifying Ingredients} \\[1mm]
    \tiny 
    1. Scrape ingredient quantities\\
    2. Standardize quantities to grams\\
    3. Manual search for non-standard measure weights
};

\node[box, anchor=north, fill=yellow!20] (quantCO2) at ([xshift=12cm] quantIngredients.north) {%
    \scriptsize\textbf{Quantifying CO$_2$-eq} \\[1mm]
    \tiny
    1. Remove insignificant ingredients\\
    2. Automated CO$_2$-eq search on healabel.com\\
    3. Manual CO$_2$-eq search for remaining ingredients\\
};

\node[box, anchor=north, fill=red!20] (quality) at ([xshift=12cm] quantCO2.north) {%
    \scriptsize\textbf{Quality Assessment} \\[1mm]
    \tiny
    1. Manual inspection on 100 randomly selected ingredients
};

\node[box, anchor=north, fill=orange!20] (greenConversion) at ([xshift=12cm] quality.north) {%
    \scriptsize\textbf{Green Conversion} \\[1mm]
    \tiny
    1. Convert CO$_2$-eqs to greenness scores
};

% Incoming arrow labeled "Food.com" into the Pre-filtering box
\draw[arrow] ([xshift=-1cm] prefilter.west) -- (prefilter.west)
    node[pos=0, left] {\footnotesize\textbf{Food.com}};

% Arrows connecting the boxes
\draw[arrow] (prefilter.east) -- (quantIngredients.west);
\draw[arrow] (quantIngredients.east) -- (quantCO2.west);
\draw[arrow] (quantCO2.east) -- (quality.west);
\draw[arrow] (quality.east) -- (greenConversion.west);

% Outgoing arrow labeled "RecipeEmission" from Green Conversion (no box)
\draw[arrow] (greenConversion.east) -- ++(1.5cm,0)
    node[pos=1, right] {\footnotesize\textbf{RecipeEmission}};
\end{tikzpicture}
% \end{document}
\end{figure}
% \end{minipage}

==> dataanalysis.tex <==


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%   STATISTIC TABLE
\begin{figure*}[!tp]
\centering
\begin{subfigure}{.33\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{Figures/user_rankvsrating.pdf}
  \caption{}
  \label{fig:sub_user_rank}
\end{subfigure}%
%
\begin{subfigure}{.33\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{Figures/item_rankvsrating.pdf}
  \caption{}
  \label{fig:sub_item_rank}
\end{subfigure}
%
\begin{subfigure}{.33\textwidth}
\centering   \includegraphics[width=1\linewidth]{Figures/rating_distro.pdf}
\caption{}
\end{subfigure}
%
%\caption{Long-tail distributions of the RecipeEmission and other datasets. (a) User engagement distribution (total ratings of each user). The RecipeEmission dataset has a similar distribution as the starting Food.com dataset and baselines. There are no users with a large number of ratings because of the filtration steps over the minimum number of interactions per item. (b) Item popularity distribution (total ratings of each item). The distribution of the RecipeEmission dataset follows closely that of the original Food.com. MovieLens datasets filter on the minumum number of interactions per user which can be noted by the trunkated distributions in this panel.}
\caption{Distribution of the statistics for the RecipeEmission and conventional datasets. \textbf{(a)} Long-tail distributions of the user engagement (total ratings of each user). RecipeEmission has a similar distribution as the starting Food.com dataset and baselines. There are no users with a large number of ratings because of the filtration steps over the minimum number of interactions per item. \textbf{(b)} Long-tail distributions of the item popularity distribution (total ratings of each item). RecipeEmission closely follows the distribution of the original Food.com. MovieLens datasets are filtered on the minimum number of interactions per user which can be noted by the truncated distributions in this panel. \textbf{(c)} Rating distribution scaled to the set $\{1, \ldots, 5\}$. All datasets but Book-Crossing have a skew towards high rating values. RecipeEmission respects the distribution of the original Food.com dataset, which follows a similar pattern as the MovieLens datasets.}
\label{fig:dataset_props}
\end{figure*}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table*}[!t]
\centering
\caption{Dataset statistics. RecipeEmission has a comparable sparsity to the baseline datasets. The reduced number of users and items is a result of the filtration steps to improve the efficiency in finding the CO$_2$-eq of the ingredients. We also see a high average rating in both RecipeEmission and Food.com, which needs to be accounted for when comparing the algorithms.}
\label{tab:dataset-comparison}
\resizebox{\textwidth}{!}{%
\begin{tabular}{l c c c c c}
\hline\hline
                                                                             & \textbf{RecipeEmission} & Food.com & Movielens100k~\cite{harper2015movielens} & Movielens1M~\cite{harper2015movielens} & Book-Crossing~\cite{ziegler2005improving} \\ 
                                                                          \rowcolor{gray!50}
\#users                                                                      & 32.090           & 226.570   & 943           & 6.040        & 105.283        \\ 
\#items                                                                      & 5.595            & 231.637   & 1.682          & 3.706        & 340.556        \\ 
\rowcolor{gray!50}
\#interactions                                                               & 247.219          & 1.132.367  & 100.000        & 1.000.209     & 1.149.780       \\ 
sparsity                                                                     & 99.86\%         & 99.998\% & 93.70\%       & 95.53\%     & 99.997\%      \\ 
\rowcolor{gray!50}
rating values                                                               & \{0,\ldots, 5\}               & \{0,\ldots, 5\}         & \{1,\ldots, 5\}              & \{1,\ldots, 5\}            & \{0,\ldots, 10\}             \\ 
average rating (std.)                                                               & 4.57 ($\pm 1.054$)           & 4.41 ($\pm 1.26$)    & 3.53 ($\pm 1.13$)          & 3.58 ($\pm 1.12$)       & 2.87 ($\pm 3.85$)         \\ 
\rowcolor{gray!50}
med. interaction per item $\backslash$ user & 27$\backslash$3              & 2 $\backslash$ 1       & 27 $\backslash$ 65            & 124 $\backslash$ 96         & 1$\backslash$1 \\
\rowcolor{gray!50}
%\begin{tabular}[c]{@{}l@{}}median interactions\\ per item $\backslash$ user\end{tabular} & 27$\backslash$3              & 2 $\backslash$ 1       & 27 $\backslash$ 65            & 124 $\backslash$ 96         & 1$\backslash$1              \\ 
\hline\hline
%\begin{tabular}[c]{@{}l@{}}median interactions \\ per user\end{tabular}      & 3               & 1        & 65            & 96          & 1             \\ \hline\hline
\end{tabular}}
\label{tab_stat}
\end{table*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In this section, we present the properties and statistics of the prepared RecipeEmission dataset.

% \smallskip
% \noindent \textbf{Outline of the methods.} Building the RecipeEmission dataset posed several challenges, such as: i) a high sparsity ($99.998\%$); ii) ingredient quantities missing or described in different ways (cups, graphs, piece); iii) no standardized and unified repository to identify the CO$_2$-eq of an ingredient; iv) CO$_2$-eq values being unknown for some ingredients. To keep the discussion concise, we outline the main steps of building the dataset in the sequel and defer the details to Sec.~\ref{subsec:buildData}. 

% \textcolor{blue}{Our approach to addressing these challenges was to retain as many interactions as possible from the original dataset while ensuring reliable CO$_2$ estimates. We also aimed to preserve the original dataset’s properties and statistical characteristics.} Thus, we proceeded in three steps. First, we filtered out recipes with a single rating to limit the search for the carbon footprint to the most relevant entries and we removed recipes for which ingredients were missing. \textcolor{blue}{This was done to ensure a high-quality subset for subsequent CO$_2$ estimation.} Second, we scraped the ingredient quantities from the website Food.com and standardized measurements to grams for ingredients originally listed in qualitative terms (e.g., pieces or a pinch). \textcolor{blue}{To achieve this, manually crowdsourced annotations were collected for around 4,000 ingredients.} Third, we quantified the CO$_2$-eq of recipes through a combination of automated and manual searches across online repositories and scientific publications.

% A quality assessment of the resulting dataset was performed in two directions. First, the dataset statistics were compared to those of the original Food.com-based dataset as shown in Fig.~\ref{fig:dataset_props} and Table~\ref{tab_stat}. Second, 100 random ingredients were taken, and their retrieved CO$_2$-eq was re-inspected, \textcolor{blue}{the annotation process and quality assessment are detailed in Sec.~\ref{subsec:buildData}}. We found an accuracy of $92\%$, whereas we observed little changes for the remaining ones. \textcolor{blue}{Finally, considering that the dataset contains many recipes with relatively low CO$_2$-eq values, we derived the greenness values by applying a logarithmic function on CO$_2$-eq values to smooth out large variations (see Eq.~\eqref{eq_greenness}). The result is a greenness distribution where larger values imply greener items.}

\subsection{Dataset statistics} 

RecipeEmission has $32.093$ users, $5.605$ recipes, and $247.521$ interactions, modelled as explicit ratings $\{0,\ldots,5\}$ leading to a sparsity of $99.86\%$. Figs.~\ref{fig:dataset_props}(a) and~\ref{fig:dataset_props}(b) show that RecipeEmission preserves key properties of conventional RecSys datasets such as the long-tail distribution of both user engagement --most user engage with few items-- and item popularity --a few items collect most ratings.

Table~\ref{tab_stat} contrasts the statistics of these datasets. RecipeEmission has fewer users, items, and interactions than Food.com. This is the result of the performed filtration steps to ease the mining the CO$_2$-eq, which also remove noisy/spurious interactions. That is, many users have a few interactions with the items, as shown also in the last row of Table~\ref{tab_stat}. Hence, we selected only recipes with at least $20$ ratings while still preserving the long-tail distribution and a sparsity greater than 99.8\%, in order to retain comparability with conventional RecSys datasets.

RecipeEmission has an average rating of $4.57$, which is close to its maximum of five. This is inherited from the ratings present in the original Food.com dataset. To illustrate the latter, Fig.~\ref{fig:dataset_props} (c) shows that the rating distributions of these two datasets and those of the baselines are similar and skewed towards higher values. Consequently, this skewness will bias the predicted recommendations towards high values. That is, the predicted ratings will have a lower spread which may lead to similar accuracies when comparing different RecSys algorithms. Thus, a relative comparison w.r.t. a baseline algorithm is more insightful to draw conclusions than focusing on absolute numbers. We shall elaborate on the latter in Sec.~\ref{sec:results}.

\begin{figure}[!tp]
\centering
\begin{subfigure}{.4\textwidth}
  \includegraphics[width=1\linewidth]{Figures/user_item_co2.pdf}
  \caption{}
  \label{fig:user_item_co2}
\end{subfigure}%
\centering
\begin{subfigure}{.4\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{Figures/user_item_greenness.pdf}
  \caption{}
  \label{fig:user_item_greenness}
\end{subfigure}%
\vspace{\floatsep}
\begin{subfigure}{.4\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{Figures/emissions_per_rating.pdf}
  \caption{}
  \label{fig:emissions_per_rating}
\end{subfigure}%
\begin{subfigure}{.4\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{Figures/greenness_per_rating.pdf}
  \caption{}
  \label{fig:greenness_per_rating}
\end{subfigure}%
\caption{Emission distributions of RecipeEmission dataset. \textbf{(a)} CO$_2$ values of users and items. The high CO$_2$-eq outliers are again the result of recipes with large quantities of high-CO$_2$ products. \textbf{(b)} greenness distributions of RecipeEmissions dataset \textbf{(c)} Distribution of emissions per rating. The large number of outliers is caused by the long-tail distribution of CO$_2$ values of recipes. \textbf{(d)} Greenness distributions over the rating values. There is no apparent distribution shift to the rating, indicating that users did not account for the item greenness when rating them.}
\label{fig:co_rank_rating}
\end{figure}


%
% \smallskip
\subsection{CO$_2$-eq distribution} 
Fig.~\ref{fig:user_item_co2} shows the CO$_2$-eq distributions of the recipes and users at the interval $[0, 200]$ Kg. Most recipes have a small footprint, and most users interact with recipes with a lower footprint. The decay of these curves indicates a long-tail CO$_2$-eq distribution similar to that of ratings. High CO$_2$-eqs are typically associated with items containing large quantities of high-CO$_2$ ingredients, such as meat products. Most recipes do not contain such high quantities, leading to a low CO$_2$-eq. Thus, the greenness of different recommender systems in absolute terms is unlikely to differ much. 
Analogously, Fig. \ref{fig:user_item_greenness} shows the greenness distribution for the recipes and users. The recipes are skewed towards greener values and, similarly, users interact mostly with greener items. 

Fig. \ref{fig:emissions_per_rating} shows the recipe CO$_2$-eq distribution w.r.t. the ratings. We observe no apparent difference between the distributions, indicating the recipes' carbon footprint plays a minor role in the ratings. 
\textcolor{blue}{This is a satisfactory observation, as the distribution of CO$_2$-eq values with respect to the distribution of rating values is unbiased, ensuring it does not interfere with our experimental analysis. For instance, if items with higher CO$_2$-eq values tended to receive higher ratings (e.g., 5 stars), the RecSys model could suffer from a positivity bias~\cite{huang2024going}, leading it to over-recommend these high-rated items. Such a bias would not only skew recommendation quality but also compromise the accuracy of our sustainability analysis by favoring certain groups of items. However, as shown in Fig.~\ref{fig:emissions_per_rating}, our data does not exhibit this correlation, allowing us to conduct both recommendation and greenness analysis without concern for bias related to CO$_2$-eq values.} \textcolor{blue}{Lastly, in Fig. \ref{fig:greenness_per_rating}, the greenness distribution w.r.t. the ratings is shown. Similarly to the CO$_2$-eq, there is no strong difference between greenness values for different ratings, indicating that users did not consider greenness when rating items.}

==> methods.tex <==

In this section, we first present the steps followed to build the RecipeEmission dataset in Sec.~\ref{subsec:buildData}. Then, in Sec.~\ref{subsec:alg}, we detail the algorithms used for benchmarking. Finally, in Sec.~\ref{subsec:data_split}, we elaborate on the data split procedure.



%SUBSECTION
\subsection{Building the Dataset}\label{subsec:buildData}


We built the RecipeEmission dataset from the Food.com (the original) dataset present in \cite{majumder2019generating} by adding the CO$_2$-eq and greenness to the different recipe items. We broke each recipe down into its ingredients (present in the original dataset) and the respective quantities (not present in the original dataset). Upon scraping the ingredient quantities and the CO$_2$-eq, we computed the recipe CO$_2$-eq as a weighted sum of those of the ingredients. This task presents the following intertwined challenges: 
%
\begin{itemize}
\item[--] \textcolor{blue}{\emph{high interaction sparsity:}} the original dataset is sparse ($99.998\%$) and often it contains a few interactions per user or item; this leads to some recipes being rated only by one user and to some users having rated only one recipe;
\item[--] \textcolor{blue}{\emph{missing ingredient quantities}} quantities of the ingredients are not present in the original dataset and need to be found differently;
\item[--] \textcolor{blue}{\emph{non-unified description:}} descriptions of the quantities differ (e.g., 1-2 cups, 1.5 grams) and they are often expressed in qualitative terms (1 piece, a pinch);
\item[--] \textcolor{blue}{\emph{lack of CO$_2$-eq consensus:}} there is no standard and unified repository to find the CO$_2$-eq of the different ingredients (this differs from the country of origin, the technology used to harvest them, transportation to destination, and season); this often requires extensive manual work;
\item[--] \textcolor{blue}{\emph{missing CO$_2$-eq values:}} CO$_2$-eqs are missing for particular ingredients, leading to recipes having only some ingredients for which the CO$_2$-eq could be found.
\end{itemize}
%
Here, we present the methods pursued to address these challenges. These methods consider the thin balance between \emph{including as many interactions as possible} and \emph{having reliable CO$_2$-eq measures} for the items. Our focal principle is to preserve the key properties [cf. Fig.~\ref{fig:dataset_props}] and statistics [cf. Table~\ref{tab_stat}] of the original dataset to ensure that they remain comparable to baselines. The methods are composed of five steps: $i)$ pre-filtering the data; $ii)$ quantifying the ingredients in the recipes; $iii)$ quantifying the CO$_2$-eq; $iv)$ quality assessment; $v)$ quantizing the CO$_2$-eq. \textcolor{blue}{Fig.~\ref{fig:dataset_building} provides a high level overview of the process of building the dataset.}

\begin{figure}
  \includegraphics[width=\textwidth]{Figures/dataset_building.pdf}
  \caption{\textcolor{blue}{Overview of the steps taken to build the dataset. First of all, pre-filtering is performed, followed by ingredient and CO$_2$-eq quantification. Finally, the CO$_2$-eq values are transformed to a greenness scale.}}
  \label{fig:dataset_building}
\end{figure}

%%%% PREFILTERING
\smallskip
\noindent\textbf{Pre-filtering.} The long-tail distribution of the Food.com dataset [cf. Fig.~\ref{fig:dataset_props}] implies that we need to find the CO$_2$-eq for some items that play a minor role in assessing the overall performance of a RecSys algorithm\footnote{These items would, however, be relevant if we were interested in addressing the (strict) cold start problem for GRS. But since our focus is on assessing the \emph{greeness} of RecSys algorithms as a whole, we can ignore these items. Typically, these interactions are treated as spurious or erroneous and are removed.}. To reduce the number of recipes for which the CO$_2$-eq has to be found, we filtered out the items and users with a few interactions as commonly done in RecSys datasets --e.g., MovieLens filters on the minimum number of interactions per user~\cite{harper2015movielens}. Specifically:
%%%%%%%
\begin{enumerate}[label=\arabic*)]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\item We removed all recipes having less than $20$ ratings.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\item From the remaining recipes, we removed those for which not all ingredients could be found.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\item Further, we removed all users that had no interaction with the remaining recipes.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\item From the recipes with more than $20$ interactions, we removed those users that have rated only that recipe, while still maintaining at least $20$ interactions per recipe.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\item {Finally, we removed those recipes for which all users have rated less than 20 recipes on average. That is, for each recipe, we extracted the user IDs of users who have interacted with the recipe and measured their total number of interactions. Then, we removed those recipe items for which the respective users rated less than 20 items. The latter helps us remove recipes that occur only in sparse parts of the dataset and tackle the cold start issues.} %\red{@Raoul: check what I wrote here based on our long-time ago discussion. I recall though there you were talking about "averages". Could you explain it here and update this part accordingly?} 
This led to the final RecipeEmissions dataset reported in Table~\ref{tab_stat}.
%
%\blue{Finally, we also removed recipes for which all users rated less than 20 recipes on average.}\red{EI: I don't get this! Does it mean we removed those recipes that had again less than $20$ ratings?} \green{Explanation: first we removed all recipes with less than 20 ratings (so less than 20 users). Later on, we removed also recipes for which its \emph{users} had less than 20 ratings \emph{on average}. In other words, we calculate the average number of interactions among users of every recipe and we remove all recipes for which this is less than 20. We discussed this a long time ago, and the main reason we did this, was to remove recipes that only occured in very sparse parts of the dataset. We figured this would be likely to not change the results much, while at the same time it would cost much to find their CO2.}\red{EI: Still unclear to me! We need to talk about this; so you can explain it to me in 5 min.} This led to the final RecipeEmissions dataset reported in Table~\ref{tab_stat}.
\end{enumerate}

%%%% QUANTIFY INGREDIENTS
\smallskip
\noindent\textbf{Quantifying ingredients.} The original dataset from \cite{majumder2019generating} does not contain the ingredient quantities, which we got from Food.com:
%%%%%%%%%%%%%%%
% ENUMERATE
\begin{enumerate}[label=\arabic*)]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\item \emph{Scrape:} We scraped Food.com using the URL:
\begin{center}
\emph{www.food.com/[tag]/[recipe name]-[recipe id]}.\smallskip\\ 
\end{center}
Here \emph{[tag]} is \emph{recipe} or \emph{about} depending on the recipe. The \emph{[recipe name]} is comprised of the decapitalized version of the recipe name with spaces replaced by hyphens (-). The \emph{[recipe id]} is also available in the original dataset.
%
All ingredients on Food.com have unique identifiers, but those do not always correspond to the identifiers in the original dataset. However, the order of ingredients on Food.com follows that in the lists. We contrasted the list lengths and the ingredient names to find the corresponding entities, and we also checked this manually for $50$ random recipes. Thus, we scraped the ingredient quantities and respective units in their default order from Food.com. \smallskip

For 797 recipes, the ingredient list on Food.com contained more ingredients than the list in the original dataset. These additional ingredients formed alternatives or minor additions that do not change the recipe. We checked if the names of the ingredients in the original dataset were contained in the names of scraped ingredients. If so, we matched the two and retrieved the respective quantities; otherwise, we considered the scraped ingredient not to be present in the original dataset and removed the ingredient.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\item \emph{Standardization:} The quantities on Food.com are expressed in different forms (e.g., range 1-2 cups; decimal format 2.5 cups; decimal fractions 2 1/2 cups) and in different units (grams, ounce, pinch). We standardized the quantities into a decimal format and in grams to allow for an easier CO$_2$-eq conversion, which is expressed in Kg. The conversion rates are reported in Table~\ref{tab:my-table-conv}.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\item \emph{Manual completion:} \textcolor{blue}{To estimate the weight of ingredient instances in non-standard quantities (e.g., "two chicken breasts," "a bunch of cabbage," or "a handful of cabbage"), we engaged four student annotators from diverse demographic and cultural backgrounds. Each annotator was tasked with determining the weight in grams of various ingredient-measure combinations sampled from our dataset. They were instructed to search for the ingredient and measure combination on Google.com and record the first relevant result they found. Additionally, they were asked to provide their source and rate their confidence in the accuracy of their findings on a scale from 1 to 10 to support the verification process. To enhance efficiency and consistency, we provided custom software that allowed annotators to input both their results and confidence levels directly. The software randomly assigned ingredient-measure combinations, and each annotator processed half of the dataset, ensuring all ingredients were annotated multiple times.}

\textcolor{blue}{Each of the 4,010 non-standard ingredient instances was annotated. Estimates with confidence ratings below 5 were re-examined, leading to 73 re-annotations. To assess inter-rater reliability, we calculated the mean absolute difference between annotations from different raters, which revealed a disagreement of a mere 2\%, indicating a high level of reliability.}
%\textcolor{red}{An annotator estimated the weights for each of the $4.010$ ingredient instances that were in non-standard quantities and with repetition (e.g., two chicken breasts, a bunch of cabbage, or a handful of cabbage) by assigning it to the first search result on Google.com. 
%We found the quantities for \blue{$4.010$} ingredients which were in non-standard quantities (e.g., two chicken breasts or one bell pepper). A manual annotator estimated the weights of each ingredient by assigning it to the first search result on Google.com. 
%Annotators also provided the source and a numerical value (1-10) of how certain they were about the correctness of the annotation. Annotations with certainties below $5$ were re-inspected, resulting in $73$ re-annotations. \textcolor{blue}{Moreover, as a measure of the inter-rater reliability, we calculated the mean absolute difference between the annotations of the different raters. This showed a mere $2\%$ disagreement between annotators, indicating a high reliability of annotations}}
\end{enumerate}

%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%% TABLE
\definecolor{Gray}{gray}{0.9}
\begin{table}[t]
\caption{Ingredient categories, their representations, and their corresponding weights conversion from pint, cup, teaspoon, and tablespoon to grams. "na." implies that measuring approach was not present for the specific category. The "pinch" metric was used for spices and salt and we choose salt as the representative ingredient with a conversion rate of 0.36 grams.}
\label{tab:my-table-conv}
\begin{tabular}{lccccc}
\hline\hline
\rowcolor{Gray}
{\textbf{Category}}     & \textbf{Represented by} & \textbf{Pint-to-g} & \textbf{Cup-to-g} & \textbf{Teaspoon-to-g} & \textbf{Tablespoon-to-g} \\
{liquids}               & water                   & 473.18   & 236.59   & 4.93 & 14.79         \\
\rowcolor{Gray}
{sugars and sweeteners} & raw sugar               & 414.02   & 227.36  & 4.74  & 14.21        \\
{flours}                & all-purpose flower      & 250.31   & 125.16 & 2.61 & 7.82         \\
\rowcolor{Gray}
{oils and fats}         & olive oil               & 434.38    & 217.66   & 4.53  & 13.6       \\
{spices}                & cinnamon                & 264.98   & 132.49  & 2.76  & 8.28         \\
\rowcolor{Gray}
{nuts}                  & almonds                 & 217.66     & 108.83  & na.  & na.       \\
{fruits and vegetables} & onion                   & 104.10  & 150    & na.  &na.      \\
\hline\hline
\end{tabular}
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%QUANTIFYING-CO2
\smallskip
\noindent\textbf{Quantifying CO$_2$-eq.} Aided by the list of ingredients, the respective quantities, and the standardized units, we found the CO$_2$-eq of the $2735$ unique ingredients as follows: %\blue{$2735$}\footnote{\red{EI: above we have 4010 ingredients in non-standard quantities but we also had other ingredients, which if I'm not wrong were quite a few? Can we give that all number somewhere? But where we say we found the co2-eq for 2735 ingredients. So, one would ask what happened to the remaining ones. We shall mention somewhere this!} \green{I am not sure I was clear here: there is a number of ingredients, i.e. 2735, but the ingredients are used in different instances. So, we have the ingredient cabbage, for example. Cabbage has a fixed greenness value per kg. But, cabbage is used in different instances (so, a pack of cabbage, a bunch of cabbage, and a handful of cabbage. That is why there are more instances (i.e... 4010 non-standard ones) than ingredients.)}} ingredients as follows:
%%%%%%%%%%%%%%%
% ENUMERATE
\begin{enumerate}[label=\arabic*)]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\item \emph{Ingredient filtration:} First, we removed $705$ ingredients present in quantities smaller than $50$ grams. These ingredients are in small relative quantities or have a low CO$_2$-eq, such as spices and flavorings \cite{marie_2022, marie_2022_2}. The threshold of $50$ grams is chosen as that of having a low impact on the whole recipe CO$_2$-eq, since in many recipes, the overall CO$_2$-eq is governed by a few ingredients present in large quantities and with a large carbon footprint (e.g., meat products).%, the threshold of $50$ grams is qualitatively chosen as that of having a relatively low impact on the whole recipe CO$_2$-eq.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\item \emph{Automated search:} We searched the CO$_2$-eq of all ingredients on healabel.com. \textcolor{blue}{This source, which provides the most extensive list of ingredients with CO$_2$-eq data, aggregates information from books, journals, and validated online articles, including the FDA's Food Resources for Consumers, the World Health Organization, and the US Department of Agriculture.} Having an extensive collection of CO$_2$-eq, this website also allowed a consistent measure across the different items in the dataset. We extracted the CO$_2$-eq via the ingredient names using the URL:
\begin{center}
\emph{https://healabel.com/ [first letter ingredient] / [ingredient name]}.
\end{center}
Multiple word names are separated with a hyphen (-). We searched ingredients both in their singular and plural forms (e.g., nut and nuts) as both were present. Several ingredients are variations of others (e.g., red pepper, green pepper) and have comparable CO$_2$-eq. So, we removed the adjectives and searched their stem form (e.g., pepper). For some composite words, the adjective represents the main ingredient (e.g., meat substitute). {However, for such ingredients, it is inaccurate to use the adjective to find the CO$_2$-eq. For example, a meat steak differs from a meat sauce. Thus, we found the CO$_2$-eqs of these ingredients manually.}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\item \emph{Manual search:} We searched the CO$_2$-eq first on healabel.com to standardize the data as much as possible and then in literature. The latter is achieved by searching on Google Scholar using the query \emph{ [ingredient name] CO$_2$ footprint} and retrieving the CO$_2$-eq from the most cited paper. The papers used for this step are \cite{yuttitham2011carbon, sevenster2008sustainable, dalla2017environmental, fantozzi2019life, parajuli2021cradle, taylor2014greenhouse, vasilaki2016water, pelletier2013carbon, espinoza2011carbon}.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\end{enumerate}

%%%%QUALITY CHECK
\smallskip
\noindent\textbf{Quality assessment.} To evaluate the quality of the dataset, $100$ random ingredients were selected, and the accuracy of their retrieved CO$_2$-eq was manually inspected. \textcolor{blue}{Due to the complexity of this process, we evaluated the similarity between the ingredient name and the corresponding name used to retrieve the CO$_2$-eq. For example, retrieving the exact CO$_2$-eq value for the ingredient "1 cup of shredded bell pepper" is a complex task, or in some cases, even impossible. Hence, we tackled this issue by retrieving the CO$_2$-eq value for the most similar ingredient to "1 cup of shredded bell pepper" with a known CO$_2$-eq. In this case, the ingredient "bell pepper" would be the best option. The resulting accuracy of this evaluation was $92\%$, indicating that for $92\%$ of the ingredients, we could accurately retrieve the CO$_2$-eq value.} We deemed this accuracy satisfactory as we are not interested in the precise CO$_2$-eq but in relative quantification. A more precise quantification should start by standardizing the quantities of the different ingredients, their densities, the dynamics of CO$_2$-eq (season, distance from the user), and the sources from which the CO$_2$-eq is retrieved. This by itself requires extensive separate research.\footnote{\textcolor{blue}{The complexity arises from the lack of global standardization in CO$_2$-eq and weight conversions for ingredients. For example, the conversion rate for \emph{a portion of beef} differs substantially between Texas and the Netherlands. Factors such as the breed and age of the animal further complicate this. Therefore, constructing a unified dataset for detailed CO$_2$-eq analysis would require extensive interdisciplinary research, which goes beyond the scope of a single paper.}}

%%%%%GREEN CONVERSION
\smallskip
\noindent\textbf{Green conversion.} Each of the above steps introduces some uncertainty to the precise CO$_2$-eq of whole recipes. Factors contributing particularly to this uncertainty include the precise weight calculation of the ingredients, manual annotations, removal of the ingredients with small quantities, variations in ingredient names, accuracy of CO$_2$-eq retrieval, and the sampling used in quality assessment. \textcolor{blue}{To reduce the effect of this uncertainty and to be consistent with the interval of rating values, we transformed the CO$_2$-eq into \emph{greenness} values at the interval $[0, 5]$, where a low value corresponds to a less green item (high CO$_2$-eq) and a high value to a greener item (low CO$_2$-eq).}
%
%The CO$_2$-eq in Kgs of the retried recipes have an uncertainty around the indicated value because of the tedious task of finding a unified way of quantifying the CO$_2$-eq. To reduce the effect of this uncertainty, we quantized the CO$_2$-eq into a discrete interval as done for explicit ratings. More precisely, we quantized the CO$_2$-eq into \emph{greenness} values in the interval $\{0,\ldots, 5\}$, where a low value indicates a less green item (high CO$_2$-eq) and a low value a greener item (low CO$_2$-eq). This greenness conversion is done so that the interval matches that of the ratings and also has a similar ascending order for a more "useful item" (high rating, high greenness). 
%
Specifically, denoting the CO$_2$-eq of item $i$ by $c_i$, the greenness $g_i$ is defined as
%
\begin{equation}\label{eq_greenness}
g_i = \ccalQ\left[\log\left(1+ \frac{1}{c_i}\right)\right]
\end{equation}
%
\textcolor{blue}{where the inverse ensures that items of low CO$_2$-eq are greener and vice versa; the logarithm amortizes the exponential decay spreading of the CO$_2$-eq; and $\ccalQ[\cdot]$ is a function that projects the greenness values into $[0, 5]$ interval, e.g., values higher than 5 are mapped to 5. We added a one within the logarithm to have only positive values inspired by the tf-idf weighting \cite{salton1988term}. This greenness conversion matches that of the ratings and has a similar ascending order for a more "useful item" (high rating, high greenness).}
%
%\blue{Another effect of the logarithm is that it also reduces the uncertainties around the found CO$_2$-eq.}


%SUBSECTION
\subsection{Algorithms}\label{subsec:alg}

We considered the following eight algorithms: \textcolor{blue}{i) \emph{random predictions} generated for all ratings in the test set;} ii) \emph{global mean} rating prediction of the training set; iii) \emph{Item nearest neighbor (ItemNN)}~\cite{sarwar2001item}; iv) \emph{User nearest neighbor (UserNN)}~\cite{resnick1994grouplens}; v) \emph{Singular value decomposition (SVD)}~\cite{sarwar2002incremental}; vi) \emph{SVD++}~\cite{koren2008factorization} that enhances SVD by accounting for implicit ratings; vii) \emph{CoClustering} \cite{george2005scalable} that uses k-means to assign similar users/items in the same cluster and uses the mean cluster rating for prediction; viii) \emph{sparse linear method (Slim)}~\cite{ning2011slim}, an ElasticNet-based neighboring approach; ix) \emph{graph neural networks {GNN}} \cite{berg2017graph} that use graph convolutions to perform the matrix completion.

%The rationale behind this choice of algorithms is as follows. 
We wanted to establish a baseline (random and global mean) that would allow a relative comparison of the conventional neighboring-based (ItemNN and UserNN), matrix factorization (SVD and SVD++) and clustering-based (CoClustering) approaches. We included Slim as an additional neighboring-based approach since it has shown a consistent performance in RecSys tasks\footnote{{https://www.amazon.science/latest-news/amazon-scholar-george-karypis-receives-icdm-10-year-highest-impact-award}}. GNNs have been considered as a more representative alternative to neighboring-based approaches since they can capture information from multi-hop neighbors. This set of algorithms has been kept simple for three reasons. First, they are the backbone of a myriad of more sophisticated solutions; hence, analyzing them will serve as a baseline for the follow-up alternatives. Second, they often achieve a comparable performance w.r.t. more complex solutions \cite{ferrari2019we}. And third, more involved deep learning solutions often require extensive hyperparameter tuning that is beyond our scope. Below, we detail their inner-working mechanism.

\smallskip
\noindent\textcolor{blue}{
\textbf{Random predictions} This method generates random predictions for all items in the test set.
}

\smallskip
\noindent\textbf{Global mean.} This method computes the global mean rating of the training set and assigns that value to the items in the test set. %It contains no hyperparameters.

\smallskip
\noindent\textbf{Item nearest neighbor (ItemNN).} This is a neighboring-based method using item-item collaborative filtering. The cosine similarity is used to find the neighboring items. We estimate the predicted rating $\hat{r}_{ui}$, between an item $i$ and a user $u$ as:
%
\begin{equation}
\hat{r}_{u i}=\frac{\sum_{j \in \ccalN^{k}(i)} \operatorname{sim}(i, j)  r_{u j}}{\sum_{v \in \ccalN^{k}(i)} \operatorname{sim}(i, j)}
    \label{eq:knn}
\end{equation}
%
where $\ccalN^{k}(i)$ is the set of $k$ neighbors to item $i$. We considered the number of neighbors in \{20, 40, 60\}.


\smallskip
\noindent\textbf{User nearest neighbor (UserNN).} This is the complementary collaborative filter of the ItemNN. We followed the same setup.

\smallskip
\noindent\textbf{SVD.} This low-rank approach approximates the user-item rating matrix and uses these latent representations to fill the missing ratings. For a user $u$ and item $i$, we use the corresponding latent feature vectors, $\mathbf{p}_u$ and $\mathbf{q}_i$ to approximate a rating $\hat{r}_{ui}$ as:
%
\begin{equation}
    \hat{r}_{ui} = b_u + b_i + \mathbf{p}_u^\top\mathbf{q}_i.
    \label{eq:IRSVD}
\end{equation}
%
We optimized for $\{20, 50, 100, 150\}$ factors, a learning rate of $\{0.1, 0.01, 0.001, 0.0001\}$, a regularization parameter of $\{0.1, 0.01, 0.001, 0.0001\}$ and training epochs of $\{20, 50, 80\}$. The optimization was done using stochastic gradient descent.

\smallskip
\noindent\textbf{SVD++.} This enhances the SVD by accounting for implicit ratings, representing that users rated items in the first place, regardless of the rating value. Let the set of items rated by user $u$ be $\ccalN(u)$ and denote the latent features also as $\bbq_i$ and $\bbp_u$. Let also $\bby_j$ be the implicit feedback for item $j \in \ccalN(u)$. Then, we predict the ratings as:
%
\begin{equation}
\hat{r}_{u i}=\mu+ b_u+b_i+\mathbf{q}_{i}^{T}\left(\mathbf{p}_{u}+|\ccalN(u)|^{-\frac{1}{2}} \sum_{j \in \ccalN(u)} \bby_{j}\right)
\label{eq:SVDpp}
\end{equation}
%
where $|\cdot|$ is the set cardinality operator. We optimized for the same parameters as regular SVD. 

\smallskip
\noindent\textbf{CoClustering.} This algorithm assigns all users and items to clusters (containing either users or items) and co-clusters (containing both users and items). Then, it uses the means of these clusters and co-clusters to predict the ratings. We used $k-$means clustering and predicted the ratings as:
%
\begin{equation}
\hat{r}_{u i}=\overline{C_{u i}}+\left(\mu_{u}-\overline{C_{u}}\right)+\left(\mu_{i}-\overline{C_{i}}\right)
\label{eq:CoClustering}
\end{equation}
%
with $\overline{C_{u i}}$ being the average rating of co-cluster $C_{u i}$, and $\overline{C_{u}}$ and $\overline{C_{i}}$ being the average ratings of clusters $C_u$ and $C_i$ respectively. We optimized for $\{3, 6, 12, 24\}$ user and item (co-)clusters and for $\{20, 50, 80\}$ epochs.
%
%
%Using k-means clustering, this algorithm assigns all users and items to clusters (containing either users or items) and co-clusters (containing both users and items) and uses the means of the clusters and co-clusters to calculate predictions according to Eq. \ref{eq:CoClustering}. \noindent Here, $\overline{C_{u i}}$ is the average rating of co-cluster $C_{u i}$, and $\overline{C_{u}}$ and $\overline{C_{i}}$ are the average ratings of clusters $C_u$ and $C_i$ respectively. We optimized for 3, 6, 12 and 24 user and item clusters and for 20, 50 and 80.
%
%\begin{equation}
%\hat{r}_{u i}=\overline{C_{u i}}+\left(\mu_{u}-\overline{C_{u}}\right)+\left(\mu_{i}-\overline{C_{i}}\right)
%\label{eq:CoClustering}
%\end{equation}

\smallskip
\noindent\textbf{Slim.} This is a linear optimization-based model using the ElasticNet principle to find sparse neighbors for each user and item. The estimated rating is computed as follows:

\begin{equation}
\hat{r}_{u i}=\mathbf{r}_{u}^{\top} \mathbf{w}_{i}
\label{eq:slim1}
\end{equation}
%
where $\mathbf{w}_{i}$ is a sparse aggregation coefficient vector. Using matrices, this model can be expressed as:

\begin{equation}
\mathbf{\hat{R}}=\mathbf{R} \mathbf{W}
\label{eq:slim2}
\end{equation}
%
where $\bbR$ is the user-item rating matrix and $\bbW$ collects all aggregation coefficients. To estimate the matrix $\mathbf{W}$, the following problem is solved:

\begin{equation}
\begin{array}{ll}
\underset{{\mathbf{W}}}{\operatorname{minimize}} & \frac{1}{2}\|\mathbf{R}-\mathbf{R W}\|_{F}^{2}+\frac{\beta}{2}\|\mathbf{W}\|_{F}^{2}+\lambda\|\mathbf{W}\|_{1} \\
\text { subject to } & \mathbf{W} \geq 0 \\
& \operatorname{diag}(\mathbf{W})=0
\end{array}
\label{eq:slim3}
\end{equation}
where the matrix $\ell_1$ norm is computed elementwise. We optimized for the regularization parameters $\beta$ and $\lambda$ in $\{0.005, 0.05, 0.5\}$.

\smallskip
\noindent\textbf{Graph neural networks.} We considered one of the first approaches used for RecSys matrix completion that is based on graph convolutions \cite{berg2017graph}. The user-item rating matrix $\bbR$ is transformed into an undirected bipartite graph connecting users to items. The edge weights of this graph correspond to the provided rating value. Then, the matrix completion task is transformed into a link prediction problem, which is solved via a graph convolution autoencoder. This autoencoder leverages convolutional GNNs to learn node-specific embeddings and subsequently decodes the latter to predict the links. We optimized for a learning rate of {0.01, 0.05, 1}, dropout ratios of {0.3, 0.5, 0.7}, and {20, 50, 80} epochs.

%The rating interactions can be considered a bipartite graph, in which users and recipes are nodes and ratings between the two as edges, where the edge weights represent the corresponding rating value. Using the method described in \cite{berg2017graph}, matrix completion can be approached as a graph link prediction problem using graph convolutional neural networks in the following way: 
%
%Let $G=(\mathbf{W}, \mathbf{E}, \mathbf{R})$ be an undirected graph, in which $u_i \in \mathbf{U}$ represent users and $v_j \in \mathbf{V}$ represents items.
%
%We can then define an encoder: 
%
%\begin{equation}
%\mathbf{Z}=f(\mathbf{X}, \mathbf{A})
%\end{equation}
%
%
%, where $\mathbf{X}$ is an $\mathbf{N} \times \mathbf{D}$ feature matrix, $\mathbf{A}$ an adjacency matrix. It generates a node embedding $\mathbf{Z}=\left[z_1^T, \ldots, z_N^T\right]^T$, which captures key features of the graph.
%
%This node embedding can then be used as input to a decoder, $\hat{\mathbf{A}}=g(\mathbf{Z})$. The decoder predicts the entries of the adjacency matrix for different node embeddings, $\left(z_i, z_j\right)$.

%SUBSECTION
%\subsection{Metric}\label{subsec:Methmetric}
%
%From a pure greenest perspective, an algorithm can be considered well-performing if it estimates higher ratings for greener items and vice-versa a low rating for non green items, irrespective of the user rating to these items. The green coefficient (GC) in \eqref{eq:GPC}, reported below for convenience, aims at measuring this principle.
%%
%\begin{equation*}
%\text{GC}=\frac{\sum_{(u,i) \in \ccalI}\left(\hat{r}_{u, i}-\bar{r}\right)\left(g_{i}-\bar{g}\right)}{\sqrt{\sum_{(u,i) \in \ccalI}\left(\hat{r}_{u, i}-\bar{r}\right)^{2}} \sqrt{\sum_{i \in \ccalI}\left(g_{i}-\bar{g}\right)^{2}}}
%\end{equation*}
%%
%The neutral rating $\bar{r}$ and greenness $\bar{g}$ ensure the GC is measured w.r.t. the scales and not biased by the dataset distributions. A positive GC is attained if the estimated rating is aligned with the and greenness; i.e., a high rating is estimated for green items or when a low rating is estimated for non green items. A negative GC is attained if the estimated rating is misaligned with  the greenness; i.e., a high rating is estimated for a non green item or a low rating is estimated for a green item. Specifically, the greener item $i$, the larger positive the difference from the average greenness of the dataset (i.e., $(g_{i}-\bar{g})\gg 0$). Then:
%%%%%
%\begin{itemize}
%\item If the estimated rating is much bigger than the mean, i.e., $\hat{r}_{u, i} \gg \bar{r}$, $\text{GC}$ attains a high positive value. This implies the algorithm is prioritising green choices.
%\item If the estimated raging is much smaller than the mean, i.e., $\hat{r}_{u, i} \ll \bar{r}$, $\text{GC}$ attains a low negative value. This implies the algorithm is \emph{not} prioritising green choices.
%\end{itemize}
%%%%%
%The opposite holds if item $i$ is not a green item, i.e., $(g_{i}-\bar{g})\ll 0$. The algorithm will be considered successful if it estimates a rating much smaller than the mean; hence, the overall $\text{GC}$ will be positively high. Note that $\text{GC}\to 0$ when $\hat{r}_{u, i} \to \bar{r}$; i.e., the algorithm is not differentiating the item w.r.t the mean rating irrespectively of its greenness value. Also $\text{GC}\to 0$ when $g_{i} \to \bar{g}$; i.e., item $i$ is not the greenest nor the worst, hence, it should not play a big role in the performance. The denominator purpose is to scale the value in the interval [-1, 1], where $-1$ indicates a low performance and $1$ a high one.
%


%SUBSECTION
\subsection{Data Split}\label{subsec:data_split}

To ensure a similar distribution and no strict cold starters, \textcolor{blue}{we created the train-test split as follows: we started with an empty test set and a training set containing all interactions. We selected an interaction at random for which both the user and item occurred at least two times in the training set. This interaction was then removed and transferred to the test set. We repeated this process until the test set contained at least $20\%$ of all interactions. Using a similar process, we built the validation set from the remaining data in the training set.}
%
{This ensures that all items in the test set also occur at least once in the training set. Users and items that occur only once in the dataset can, therefore, not occur in the test set. Also, the random picking strategy makes it possible that not all users and items occur in the test set. The distribution of the ratings and greenness of the splits is shown in Fig. \ref{fig:recipe_entry}}.

\begin{figure}
  \includegraphics[width=\textwidth]{Figures/train_test_val_ful.pdf}
  \caption{Rating and greenness distributions of the training, validation and testing splits and the full datasets. Sparsities are 99.9\%, 99.9\%, 99.9\% and 99.9\% respectively.}
  \label{fig:recipe_entry}
\end{figure}



